DenoDet: Attention as Deformable Multi-Subspace Feature Denoising for Target Detection in SAR Images

Synthetic Aperture Radar (SAR) target detection has long been impeded by inherent speckle noise and the prevalence of diminutive, ambiguous targets. While deep neural networks have advanced SAR target detection, their intrinsic low-frequency bias and static post-training weights falter with coherent noise and preserving subtle details across heterogeneous terrains. Motivated by traditional SAR image denoising, we propose DenoDet, a network aided by explicit frequency domain transform to calibrate convolutional biases and pay more attention to high-frequencies, forming a natural multi-scale subspace representation to detect targets from the perspective of multi-subspace denoising. We design TransDeno, a dynamic frequency domain attention module that performs as a transform domain soft thresholding operation, dynamically denoising across subspaces by preserving salient target signals and attenuating noise. To adaptively adjust the granularity of subspace processing, we also propose a deformable group fully-connected layer (DeGroFC) that dynamically varies the group conditioned on the input features. Without bells and whistles, our plug-and-play TransDeno sets state-of-the-art scores on multiple SAR target detection datasets. The code is available at https://github.com/GrokCV/GrokSAR.

==> contents/1-taes-authors-single.tex <==
% !TEX root = ../main.tex

% author names and IEEE memberships
\author{
  Yimian~Dai,
  Minrui~Zou,
  Yuxuan~Li,
  Xiang~Li,
  Jian~Yang,
  Kang~Ni
  \thanks{
    This work was supported by
    % 国基
    the National Natural Science Foundation of China
    (62301261, % 我
    62206134, % 翔哥
    62101280, % 倪康
    62361166670), % 杨健老师
    % 省基
    the Natural Science Foundation of Jiangsu Province (BK20210588),
    % 博后面上
    the China Postdoctoral Science Foundation
    (2021M701727, % 我
    2023M731781), % 倪康     
    \emph{The first two authors contributed equally to this work. (Corresponding author: Jian Yang and Kang Ni)}
    }


  % 南理工
  \thanks{
    Yimian Dai and Jian Yang are with PCA Lab, Key Lab of Intelligent Perception and Systems for High-Dimensional Information of Ministry of Education, and Jiangsu Key Lab of Image and Video Understanding for Social Security, School of Computer Science and Engineering, Nanjing University of Science and Technology, Nanjing, China.
    (e-mail:
    \href{mailto:yimian.dai@gmail.com}{yimian.dai@gmail.com};    
    \href{mailto:csjyang@mail.njust.edu.cn}{csjyang@mail.njust.edu.cn}).
  }



  % 南邮
  \thanks{
    Minrui Zou and Kang Ni are with Nanjing University of Posts and Telecommunications, Nanjing, China. Kang Ni is also with Key Laboratory of Radar Imaging and Microwave Photonics, Nanjing University of Aeronautics and Astronautics, Ministry of Education, Nanjing, China.
    (e-mail:
    \href{mailto:traveler\_wood@163.com}{traveler\_wood@163.com};
    % \href{mailto:zhengzz\_js@126.com}{zhengzz\_js@126.com};
    \href{mailto:tznikang@163.com}{tznikang@163.com}).
  }

    % 南开
    \thanks{Yuxuan Li and Xiang Li are with VCIP, CS, Nankai University. (e-mail:
    \href{mailto:yuxuan.li.17@ucl.ac.uk}{yuxuan.li.17@ucl.ac.uk};
    \href{mailto:xiang.li.implus@nankai.edu.cn}{xiang.li.implus@nankai.edu.cn}).
    }
}
